Diffusion Models are Minimax Optimal Distribution Estimators

While efficient distribution learning is no doubt behind the groundbreaking success of diffusion modeling, its theoretical guarantees are quite limited. In this paper, we provide the first rigorous analysis on approximation and generalization abilities of diffusion modeling for well-known function spaces. The highlight of this paper is that when the true density function belongs to the Besov space and the empirical score matching loss is properly minimized, the generated data distribution achieves the nearly minimax optimal estimation rates in the total variation distance and in the Wasserstein distance of order one. Furthermore, we extend our theory to demonstrate how diffusion models adapt to low-dimensional data distributions. We expect these results advance theoretical understandings of diffusion modeling and its ability to generate verisimilar outputs.

==> trash.tex <==
% \begin{lemma}\label{Lemma:Smooth2}
%     For $k\in \Z_+$, there exists a constant $\ConstDifBoundB$ depending only on $d$ such that
%     if $p_t(x) \geq \frac{\epsC}{m_t^d}$, then
%     \begin{align}
%         \|\pd_{t} \nabla \log p_t(x)\| \leq \frac{\ConstDifBoundB\log \epsC^{-1}}{t^{3/2} \land 1}
%     \end{align}
%     holds for $0<\epsC<\frac12$.
% \end{lemma}
% \begin{proof}
% % In the following proof we abbreviate $\sigma_t$ and $m_t$ as $\sigma$ and $m$, respectively.
%     We can see that the following holds:
%     \begin{align}\label{eq:LemmaSmoothness2-1}
%       \pd_{\sigma_t} \nabla \log p_t(x)
%       &  =
%       \frac{1}{\sigma_t^2}\cdot \frac{g_1(x)}{g_2(x)} - \frac{1}{\sigma_t} \cdot\frac{g_2(x)  \int \frac{x-m_t y}{\sigma_t^{d+1}(2\pi)^\frac{d}{2}}\left(\frac{-(d+1)}{\sigma_t} + \frac{\|x-m_t y\|^2}{\sigma_t^3} \right)f(y)\exp\left(-\frac{\|x-m y\|^2}{2\sigma_t^2}\right) \dy}{g_2^2(x)}
%       \\ & \quad + \frac{1}{\sigma_t}\cdot \frac{g_1(x)\int \frac{1}{\sigma_t^{d}(2\pi)^\frac{d}{2}}\left(\frac{-d}{\sigma_t} + \frac{\|x-m y\|^2}{\sigma_t^3} \right)f(y)\exp\left(-\frac{\|x-m_t y\|^2}{2\sigma_t^2}\right) \dy}{g_2^2(x)}
%         .
%     \end{align}
%     Moreover, 
%     \begin{align}\label{eq:LemmaSmoothness2-2}
%       \pd_{m_t} \nabla \log p_t(x)
%       &  =
%       -\frac{1}{\sigma_t} \cdot\frac{g_2(x)  \int \frac{1}{\sigma_t^{d}(2\pi)^\frac{d}{2}}\left(-\frac{y}{\sigma_t} - \frac{(x-m_t y)\sum_{i=1}^d 2(m_t y_i - x_i)}{2\sigma_t^3}\right)f(y)\exp\left(-\frac{\|x-m_t y\|^2}{2\sigma_t^2}\right) \dy}{g_2^2(x)}
%       \\ & \quad +
%         \frac{1}{\sigma_t} \cdot\frac{g_2(x)  \int \frac{1}{\sigma_t^{d}(2\pi)^\frac{d}{2}}\left( - \frac{\sum_{i=1}^d 2(m_t y_i - x_i)}{2\sigma_t^2}\right)f(y)\exp\left(-\frac{\|x-m_t y\|^2}{2\sigma_t^2}\right) \dy}{g_2^2(x)}
%     \end{align}
%     In the same way as that for \eqref{eq:LemmaSmoothness-5} and \eqref{eq:LemmaSmoothness-6}, when $g_2(x) \geq \frac{\epsC}{m^d}$, \eqref{eq:LemmaSmoothness2-1} and \eqref{eq:LemmaSmoothness2-2} is bounded by 
%     $
%         \frac{C_1\log \epsC^{-1} }{\sigma^{2}}
%     $, where $C_1$ is some constant dependent on $d$.

%     Moreover, since $m_t = \exp(-\int_0^s \beta_s \ds )$ and $\sigma_t = \sqrt{1 -\exp(-2\int_0^s \beta_s \ds )}$, 
%     $|\frac{\pd m_t}{\pd t}| = |\beta_t \exp(-\int_0^s \beta_s \ds )| \leq \betahigh$ and $|\frac{\pd\sigma_t}{\pd t}| = |\frac{2\beta_t \exp(-2\int_0^s \beta_s \ds )}{\sqrt{1 -\exp(-2\int_0^s \beta_s \ds )}}| \leq \Ord(1/\sqrt{t})$ hold for $t\leq 1$.
%     In addition, $\sigma = \Ord(\sqrt{t})$ for $t\leq 1$.
%     Therefore, finally $\pd_t \nabla \log p_t(x)$ is bounded by $C(t^{-3/2}\lor 1)\log \epsC^{-1}$ for some constant depending on $d$, $\betalow$, and $\betahigh$.
% \end{proof}

In the next two lemmas, we show that we only need to approximate $\nabla \log p_t(x)$ within some bounded region.
\begin{lemma}\label{Lemma:Decay1}
    Let $0<\eps<\frac12$ and $C$ is a constant depending on $d$  and $\ConstDensityBoundE$.
    For any $t>0$, we let $A^t = [C\sqrt{\log \eps^{-1}}, C\sqrt{\log \eps^{-1}}]^d$.
    Then, we have the following: 
    \begin{align}
        \int_{x\in A^t} p_t(x) \|\nabla \log p_t(x)\|\dx \leq 
        .
    \end{align}
\end{lemma}
\begin{proof}
    Let $\|x\|^2 = r$.
    Note that the lower and upper bounds on $p_t(x)$ can be derived by considering the case when $p_0(x)$ corresponds to a Dirac measure $\delta(x\in x_*)$ for some $x_*\in [-1,1]^d$.
    When $x_*$ is farthest away from $x$, this gives the lower bound, and vice versa.
    Thus, we have that
    \begin{align}
      \frac{1}{\sigma_t^{d}(2\pi)^\frac{d}{2}}\exp\left(-\frac{r(x)+d}{2\sigma_t^2}\right) \leq  p_t(x) \leq \frac{1}{\sigma_t^{d}(2\pi)^\frac{d}{2}}\exp\left(-\frac{(r(x) - d)_+}{2\sigma_t^2}\right).
    \end{align}
      In order to have $(r(x) - d)/(2\sigma_t^2) \geq \log (\frac{1}{\sigma_t^{d}(2\pi)^\frac{d}{2}}\cdot \eps^{-1})$ holds for all $r(x)>C^2\log \eps^{-1}$, it suffices to take $C=\Ord_d(1)$.
      In other words, with this choice of $C$, we have that $p_t(x)\leq \eps$ for any $x\in \R^d \setminus A^t$.

    According to \cref{Lemma:Smooth1}, for $x$ with $r=r(x)$, we have 
    \begin{align}
    \|\nabla \log p_t(x)\| &\leq \frac{C_1|\log (m_t p_t(x))^{-1}|^\frac12}{\sigma_t}
    \\ & 
    \leq \frac{C_1\log^\frac12 (m_t)}{\sigma_t}
    \end{align}
    
    We rewrite this density bounds with respect to $r$:
    \begin{align}
           \frac{r^{d/2-1}}{\sigma_t^{d}2^{d/2}\Gamma(d/2)}\exp\left(-\frac{r(x)+d}{2\sigma_t^2}\right) \leq  p_t(r) \leq \frac{r^{d/2-1}}{\sigma_t^{d}2^{d/2}\Gamma(d/2)}\exp\left(-\frac{(r(x) - d)_+}{2\sigma_t^2}\right).
    \end{align}
  
    
    Then, for any $x\in \R^d \setminus A^t$, we have 
    \begin{align}
    \|\nabla \log p_t(x)\| \leq \frac{1}{2}
      \frac{1}{\sigma_t^{d}(2\pi)^\frac{d}{2}}\exp\left(-\frac{r(x)+d}{2\sigma_t^2}\right) \leq  p_t(x) \leq \frac{1}{\sigma_t^{d}(2\pi)^\frac{d}{2}}\exp\left(-\frac{(r(x) - d)_+}{2\sigma_t^2}\right).
    \end{align}
\end{proof}

% Next we evaluate the scale of $p_t(x)$ and $\nabla \log p_t(x)$.
% \begin{lemma}\label{Lemma:Smooth3}
%     For any  $t>0$ and $z>0$, we let $A^z = \{x\in \R^d \|x\|_\infty = m_t+z/\sigma_t\}$ and $C$ be some constant depending on $d$ and $\ConstDensityBoundE$.
%     Then, $p_t(x)$ and $\nabla \log p_t(x)$ for $x\in A^z$ is evaluated as follows:
%     \begin{align}
%         p_t(x) \leq \frac{\ConstDensityBoundE}{2m_t} e^{-z^2/2},
%         \quad
%         \|\nabla \log p_t(x) \| \leq \frac{z C\log^\frac12 m_t^{-1}}{\sigma_t}.
%     \end{align}
%     Therefore, if we use $\hat{}$
% \end{lemma}
% \begin{proof}
%     Choose $i^* $ from $ \{1,2,\cdots,d\}$ such that $|x_{i^*}| =m_t+z/\sigma_t$ holds.
%     \begin{align}
%          p_t(x) &= 
%         \int \frac{1}{\sigma^{d}(2\pi)^\frac{d}{2}}f(y)\exp\left(-\frac{\|x-m y\|^2}{2\sigma_t^2}\right) \dy
%         \\ & 
%          \leq \ConstDensityBoundE \prod_{i=1}^d  \int_{y_i \in [-1,1]} \frac{1}{\sigma(2\pi)^\frac{1}{2}}\exp\left(-\frac{(x_i-m y_i)^2}{2\sigma_t^2}\right) \dy
%            \\ & 
%          = \ConstDensityBoundE \int_{y_{i^*} \in [-1,1]} \frac{1}{\sigma(2\pi)^\frac{1}{2}}\exp\left(-\frac{(x_{i^*}-m y_{i^*})^2}{2\sigma_t^2}\right) \dy
%          \\ &
%          \leq \frac{\ConstDensityBoundE}{m_t} \int_{a=z/\sqrt{2}}^\infty \frac{1}{\sqrt{\pi}}\exp\left(-a^2\right) \dy
%            \\ &
%          \leq \frac{\ConstDensityBoundE}{2m_t} e^{-z^2/2},
%     \end{align}
%     where we used $\int_z^\infty e^{-a^2} \mathrm{d}a \leq e^{-z^2} $ \citep{chang2011chernoff} for the last inequality.

% %     On the other hand, 
% %     \begin{align}
% %          p_t(x) &= 
% %         \int \frac{1}{\sigma^{d}(2\pi)^\frac{d}{2}}f(y)\exp\left(-\frac{\|x-m y\|^2}{2\sigma_t^2}\right) \dy
% %         \\ & 
% %          \geq \ConstDensityBoundE^{-1} \prod_{i=1}^d  \int_{y_i \in [-1,1]} \frac{1}{\sigma(2\pi)^\frac{1}{2}}\exp\left(-\frac{(x_i-m y_i)^2}{2\sigma_t^2}\right) \dy
% %            \\ & 
% %          = \ConstDensityBoundE \left(\int_{y_{i^*} \in [-1,1]} \frac{1}{\sigma(2\pi)^\frac{1}{2}}\exp\left(-\frac{(x_{i^*}-m y_{i^*})^2}{2\sigma_t^2}\right) \dy\right)^d
% %          \\ &
% %          \geq \frac{\ConstDensityBoundE}{m_t^d} \left(\int_{a=z/\sqrt{2}}^{z/\sqrt{2}+\sqrt{2}m_t/\sigma_t} \frac{1}{\sqrt{\pi}}\exp\left(-a^2\right) \dy\right)^d
% %            \\ &
% %             \leq
% %            \begin{cases}
% % & \frac{\ConstDensityBoundE}{2m_t} \left(\frac12 e^{-z^2/2} - e^{-(z/\sqrt{2}+\sqrt{2}m_t/\sigma_t)^2}\right) \geq C' \exp\left(-z^2/2\right)\quad (m_t/\sigma_t = \Omega(1))
% % \\ &C' \exp\left(-z^2/2\right) \quad (m_t/\sigma_t = o(1))
% %            \end{cases}
% % \\ &  = C' \exp\left(-z^2/2\right)
% %     \end{align}
% %     for some constant $C'$
    

%     Then, we apply \cref{Lemma:Smooth1} with $\eps = \frac{\ConstDensityBoundE m_t^{d-1}}{2} e^{-z^2/2}$ to obtain that
%     \begin{align}
%         \|\nabla \log p_t(x) \| \leq \frac{z C\log^\frac12 m_t^{-1}}{\sigma_t}
%     \end{align}
%     for some constant $C$.
% \end{proof}
